Privacy Amplification via Shuffling: Unified, Simplified, and Tightened

The shuffle model of differential privacy provides promising privacy-utility balances in decentralized, privacy-preserving data analysis. However, the current analyses of privacy amplification via shuffling lack both tightness and generality. To address this issue, we propose the \emph{variation-ratio reduction} as a comprehensive framework for privacy amplification in both single-message and multi-message shuffle protocols. It leverages two new parameterizations: the total variation bounds of local messages and the probability ratio bounds of blanket messages, to determine indistinguishability levels. Our theoretical results demonstrate that our framework provides tighter bounds, especially for local randomizers with extremal probability design, where our bounds are exactly tight. Additionally, variation-ratio reduction complements parallel composition in the shuffle model, yielding enhanced privacy accounting for popular sampling-based randomizers employed in statistical queries (e.g., range queries, marginal queries, and frequent itemset mining). Empirical findings demonstrate that our numerical amplification bounds surpass existing ones, conserving up to $30\%$ of the budget for single-message protocols, $75\%$ for multi-message ones, and a striking $75\%$-$95\%$ for parallel composition. Our bounds also result in a remarkably efficient $\tilde{O}(n)$ algorithm that numerically amplifies privacy in less than $10$ seconds for $n=10^8$ users.

==> response.tex <==
%\nobalance
\clearpage
\setcounter{page}{1}

\twocolumn[
%\vspace*{1.5em}
\section*{\huge \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ Response to Reviewer Comments}
\vspace*{2em}
]


We would like to thank the reviewers for their insightful comments, which have been instrumental in enhancing the quality of our manuscript. Our responses to the observations made by the reviewers are outlined below. Modifications made to the manuscript are highlighted in {\color{blue} blue} for ease of identification.

%First of all, we would like to express our thanks to the reviewers for their comments. These comments are all valuable and very helpful for revising and improving our paper. The main responses to the meta reviewer's and three reviewers’ comments are itemized as follows. In the attached paper the changes are highlighted in {\color{blue} blue}.

\section*{Response to Meta Reviewer}

\begin{mybox}{Meta Reviewer-Item 1}
The authors should provide more intuitions to make the theoretical part easier to follow.
\end{mybox}

We would like to thank the reviewers for the feedback. To address this issue, we clarified our method in Section 4 by explaining how it uses mixture decomposition of local randomizers, as found in the privacy literature, to enhance privacy. This approach shows that shuffled random messages can appear as if from one user, increasing privacy, and that a user's randomizer outputs have a consistent distribution pattern. We have refined our analysis by focusing on specific properties of local randomizers and introduced a `probability ratio' to measure how well other users' data can mimic a specific user's data, making our privacy amplification analysis more precise and understandable. The modifications are as follows:

\begin{quote}
Our approach leverages the mixture decomposition of local randomizers, as introduced in the privacy blanket \cite{balle2019privacy} and clone reduction \cite{feldman2022hiding,feldman2023stronger} literature. The mixture decomposition of local randomizers reveal two important facts: (1) randomized and anonymously shuffled messages from other users can mimic as the message from a particular (victim) user with some probability, which are termed as blanket messages in \cite{balle2019privacy} and clones in \cite{feldman2022hiding,feldman2023stronger} and can thus amplify privacy; (2) for the local randomizer of the victim user that pertain to some properties (e.g., $(\epsilon,0)$-LDP), the probability distribution of outputs given arbitrary inputs share some resemblance. The key to analyzing tighter shuffle privacy amplification would be characterizing more concise mimic probability from other users and the probability resemblance of the victim's outputs. Compared to existing results, our framework achieves a highly precise mixture decomposition by utilizing both $(0,\delta)$-LDP and $(\epsilon_0, 0)$-LDP properties of local randomizers to capture the the probability resemblance of victim's outputs (over differed inputs), and introduces the probability ratio as simple yet effective indicates to the mimic power from other users.
\end{quote}

To more clearly articulate the theoretical foundations regarding privacy amplification lower bounds, we have updated the introductory explanation of our approach in Section 5:

%For theoretical results about privacy amplification lower bounds, we now revise the basis idea explanation of our approach at the start of Section 5 as follows:

\begin{quote}
Aiming at maximizing the divergence in observable shuffled messages given two neighboring datasets, our approach involves selecting elements $y\in \dom{Y}$ in the message space where the probabilities $\mathbb{P}[\mech{R}(x_1^0)=y]$ and $\mathbb{P}[\mech{R}(x_1^1)=y]$ differ. We then choose the worst-case data $x^*\in \dom{X}$ for other users to maximize the \emph{expected} probability ratio over differed elements, and finally, we observe the number of occurrences of these differing elements in shuffled messages. For succinctness, we summarize the occurrences of these elements and summarize them into two binomial counts, similar to the technique used in Theorem \ref{the:reduction}. The resulting amplification lower bound is presented in Theorem \ref{the:lowerbound}, indicating the (worst-case) divergence of shuffled messages is lower bounded by the divergence between two binomial counts $P_{p_0,\beta}^{q_0,q_1}$ and $Q_{p_0,\beta}^{q_0,q_1}$.
\end{quote}


\begin{mybox}{Meta Reviewer-Item 2}
The scope of this work seems to be narrow. Please make a justification.
\end{mybox}

% The shuffle model of DP, as a new paradigm (as comparision to the curator and local models) for data collecting and analyses, has show promising results for database queries and machine learning, and has been deployed in Google \& Apple's Exposure Notification Privacy-preserving Analytics [xx]. Due to its advantages over existing paradigms, it is fastly spreading to numerious domains beyond the seminal theoretical community, such as information security \cite{}, mobile/edge network, database/data mining, machine learning. With the help of this work, it has the potential to spread to many more application domains.

% This work largely advances the critical component in the shuffle model: analyzing privacy amplification via shuffling, in terms of both tightness, usability and efficiency, and can benefits both theorists and practioners in related domains. 

% For theorists, 

% (1) Our proof introduces novel and stimulating techniques. Specifically, we leverage total variation parameter to implicitly construct the mixture decomposition in Lemma A.2. This method is intuitive and yields exactly tight decompositions for various randomizers. For these randomizers where this decomposition is not tight, there is potential for extension to multi-level of  (as detailed in the Limitations section of the Appendix). Moreover, deriving the divergence inequality for cases  (e.g., in privacy amplification analyses of metric LDP mechanisms) and (e.g., in multi-message shuffle protocols) necessitate intricate analyses with the data processing inequality.

% (2) Our results shows qualitative improvements over existing LDP results (as demonstrated in Table 1) and generalize to multi-message cases (which is preferable to provide much better utility performance \cite{}). 

% (3) We provide novel constructions to establish lower bounds of privacy amplification via shuffling, which are useful to understand the limits of shuffle privacy amplfication.

% For practitioners:

% (1) The induced tighter nuermical amplfication results will directly improve privacy-utility trade-offs of existing works (e.g., ) in this area. Moreover, our algorithm is much faster than existing approaches, thus are suitable for large scale user sensitive data collecting (e.g., service usage telemetry of millions/billions users in Google/Apple/Microsoft/Meta services).

% (2) For multi-message shuffle protocols, to the best of our knowledge, no existing work provides computational methods for privacy amplification. With our tight numerical privacy amplification bound, SOTA multi-message protocols [x][x][x][x][x], listed in Table 2, can achieve much better utility and message complexity performance under a given global privacy target, thus narrowing their gap with centralized DP. In general, our framework helps multi-message shuffle protocols to achieve much better privacy-utility-message complexity trade-offs.

% (3) The derived asymptotic amplfication results that connects the amplified privacy with simple randomizer parameterizations, can help protocol designer to intuitively understand the performance of their designs and motivate the optimized hyperparameters. 

%We appreciate the opportunity to clarify the scope and significance of our work. The shuffle model of DP, a novel paradigm compared to curator and local models, has demonstrated promising results in diverse fields, including its deployment in major projects like Google \& Apple's Exposure Notification Privacy-preserving Analytics. Its rapid adoption beyond theoretical circles into domains like information security, mobile/edge networks, and machine learning attests to its broad potential.

%Our contribution significantly enhances the shuffle model's primary function - privacy amplification analysis - impacting both theory and practice:

We are grateful for the chance to elaborate on the impact and breadth of our research. The shuffle model of DP stands as a relatively new paradigm when compared to traditional curator and local models, yet it has already shown considerable promise across various applications. This includes advancements in SQL queries \cite{balle2020private,ghazi2020fewer,ghazi2021differentially,feldman2022hiding,cheu2022differentially}, federated learning \cite{girgis2021shuffled,girgis2021shuffledtradeoffs}, bandit learning \cite{tenenbaum2021differentially,garcelon2022privacy} and its deployment in major projects like Google \& Apple's Exposure Notification Privacy-preserving Analytics. Its swift integration into practical fields like database queries, information security, and machine learning underscores the model's vast applicability and potential. 
The expansive applications of the shuffle model necessitate an urgent development of a unified and efficient framework that addresses both the theoretical complexities of analyzing shuffle protocols and the practical challenges in their design and implementation, highlighting the critical needs of both theorists and practitioners.
%On the other hand, its broad applications call for a unified, tight, and fast framework for removing barriers in analyzing shuffle protocols (from theorists' perspectives) and in designing/implementing shuffle protocols (from practitioner's views).

The challenge of analyzing privacy amplification in the shuffle model of DP, as discussed in previous leading publications \cite{erlingsson2019amplification,balle2019privacy,feldman2022hiding,feldman2023stronger}, is pivotal. Nonetheless, existing works have not established sufficiently tight bounds for broader communication scenarios, limiting its applicability in real-world big data applications.
%The most important and challenging part of the increasing popular shuffle model of DP is the analyses of privacy amplification via shuffling (as pursued in a series of works \cite{erlingsson2019amplification,balle2019privacy,feldman2022hiding,feldman2023stronger} from top venues), which disguises itself from the classical local and curator models of DP. 

To summarize, we significantly enhanced the analysis of shuffle privacy amplification for the theorists and the practitioners:

For the theorists:
\begin{itemize}
\item Our innovative proof techniques, such as leveraging the total variation parameter for mixture decomposition (Lemma \ref{lemma:mixture}), lead to precisely tight decompositions for various randomizers and potential multi-level extensions.
\item We achieve qualitative advancements over existing LDP results (see Table \ref{tab:bounds}) and broaden the scope to multi-message scenarios, which are critical for improved utility.
\item New methodologies for establishing lower bounds in shuffle privacy amplification are introduced, enriching theoretical understanding.
\end{itemize}

For the practitioners:
\begin{itemize}
\item The refined numerical amplification results we offer will directly enhance the privacy-utility trade-offs in existing applications, especially in large-scale data collection scenarios.
\item Our work fills a gap in multi-message shuffle protocols by providing $\tilde{O}(n)$ computational methods for privacy amplification, as evidenced in Algorithm \ref{alg:upperbound} and Table \ref{tab:parametersmulti}. This narrows the gap with centralized DP and improves overall protocol efficacy.
\item Lastly, our asymptotic amplification findings help protocol designers grasp and optimize their designs through simplified randomizer parameterizations.
\end{itemize}

Our work not only has direct applications to existing DP randomizers and protocols  (e.g., for heavy hitter estimation \cite{qin2016heavy, bassily2017practical, wang2019locally}, multi-dimensional data publication \cite{ren2018lopub, wang2019collecting, wang2019answering}, frequent itemset mining \cite{wang2018locally}, range queries \cite{cormode2019answering}, marginal queries \cite{cormode2018marginal}, data synthesis \cite{zhang2018calm, wangT2019locally}, and machine learning \cite{jagannathan2009practical,xin2019differentially,fletcher2019decision}.), but also can motivate new multi-message protocols, as elaborated in Discussion on variation-ratio parameters at Page 8 and in the discussion of generality for shuffle protocols (which have best privacy-utility balances):

\begin{quote}
\textbf{Discussion on variation-ratio parameters.} 
The research on parameters \(p\), \(\beta\), and \(q\) shows patterns that help design protocols for the shuffle model.
Single-message shuffle protocols that utilize $\epsilon_0$-LDP randomizers are limited to $q=p=e^{\epsilon_0}$. Therefore, the clone probability $2r=2\beta p/((p-1)q)$ decreases significantly with $\epsilon_0$, and larger population are required to achieve global $(\epsilon,\delta)$-DP. Randomization mechanisms with better utility in the local model often fully exploit privacy constraints and have larger total variation bounds $\beta$, resulting in weaker privacy amplification effects (e.g., comparing randomized response with binary RR on $2$ options). Multi-message shuffle protocols typically set $q<p$ or even $q\ll p$ to increase the clone probability and reduce the number of messages transmitted per user. For local metric $d_{\dom{X}}$-DP randomizers that handle large data domains, $d_{max}$ is often set relatively high, and thus $q\geq p$. When a global privacy target is given, they need to strike a balance between local data utility (which increases with $d_{max}$) and privacy amplification effects (which decrease with $d_{max}$).
\end{quote}

\begin{quote}
\textbf{Discussion on the  generality of our framework for multi-message protocols. } We note that our framework applies to all single-message shuffle protocols with local $\epsilon$-DP or local metric DP randomizers. While for multi-message protocols in the shuffle model, based on the correlation between outputted messages, they can be primarily categorized into three main types:
\begin{itemize}
    \item[I.] The first type of multi-message shuffle protocols is achieved by invoking multiple single-message protocols. This is seen as in the Recursive protocol in \cite{balle2020private} and the utility-complexity balanced protocol in \cite{girgis2023distributed}.
    \item[II.] The second type involves sending one input-dependent message and multiple independent blanket messages, as seen in \cite{balcer2020separating,balcer2021connecting,cheu2022differentially,luo2022frequency,li2023privacy}.
    \item[III.] The third type involves sending multiple correlated messages per user. Protocols falling in this category include \cite{ghazi2020private,ghazi2021differentially} and the secret-sharing-style IKOS protocol in \cite{balle2020private}.
\end{itemize}
We also envision that there can be multi-message protocols that combines Types I and II, by invoking several protocols each is a multi-message one. Our variation-ratio framework is compatible with protocols categorized under Type I and/or Type II.    
\end{quote}

In summary, our work not only have direct applications to existing privacy preserving  protocols for well-studied data collecting/analyzing topics, but also removed the key obstacle of the new model of DP when spreading to new topics in broad application domains (including privacy-related DB researches), and can motivate novel randomizers/protocols design therein.

% For theorists:
% \begin{itemize}
% \item Our innovative proof techniques, such as leveraging the total variation parameter for mixture decomposition (Lemma A.2), lead to precisely tight decompositions for various randomizers and potential multi-level extensions (see Appendix's Limitations section).
% \item We achieve qualitative advancements over existing LDP results (Table 1) and broaden the scope to multi-message scenarios, which are critical for improved utility.

% \item New methodologies for establishing lower bounds in shuffle privacy amplification are introduced, enriching theoretical understanding.
% \end{itemize}

% For practitioners:
% \begin{itemize}
% \item The refined numerical amplification results we offer will directly enhance the privacy-utility trade-offs in existing applications, especially in large-scale data collection scenarios.
% \item Our work fills a gap in multi-message shuffle protocols by providing $\tilde{O}(n)$ computational methods for privacy amplification, as evidenced in Table 2. This narrows the gap with centralized DP and improves overall protocol efficacy.
% \item Lastly, our asymptotic amplification findings help protocol designers grasp and optimize their designs through simplified randomizer parameterizations.
% \end{itemize}



% \begin{mybox}{Meta Reviewer-Item 3}
% The main contribution of this work is theoretical. Please highlight the novelty and contribution.
% \end{mybox}

% We would like to emphasize that we contribute both theory and practice to the field of data privacy preservation within the newly emerging shuffle model of DP. 

% \begin{itemize}
% \item Theoretically, we propose new parameteization and novel techniques to analyze the privacy amplfication bounds (see Section 5), the resulting analytical bounds significantly surpass existing approaches. Specifically for SQL queries that involving with multiple analyzing targets, we employ our new framework and derives much tighter amplification results to improve privacy-utility trade-offs.
 
% \item Practically, we present an efficient numerical algorithm for privacy amplification analyses, which can scale to billions of users encountered in user data telemetry (e.g., in Google/Apple/Microsoft/Meta services), and are lacking in the multi-message shuffle model literature (and hinders the spread of shuffle model from theoretical computer science venues like STOC and SODA to other application domains, such as database/data mining, mobile/edge computing, and federated learning)
% \end{itemize}

\begin{mybox}{Meta Reviewer-Item 3}
The main contribution of this work is theoretical. Please highlight the novelty and contribution.
\end{mybox}

We thank the reviewers for recognizing our theoretical contributions. Our research also significantly improves practical applications by ensuring large databases maintain functionality after Differential Privacy (DP) implementation. This advancement supports sectors like database/data mining, mobile/edge computing, and federated learning (e.g., in \cite{erlingsson2019amplification,balle2019privacy,feldman2022hiding,feldman2023stronger}), which require complex SQL queries with minimal added noise. Previously, the lack of a scalable \(\tilde{O}(n)\) numerical algorithm for comprehensive and precise privacy amplification analysis hindered these applications. Our research addresses this by improving the balance between privacy, utility, and message complexity in shuffle protocols, bridging a vital gap in multi-message shuffle model studies that lacked a numerical method for accurate privacy calculations.

% Thank you for highlighting this aspect. Our work significantly contributes to both the theoretical framework and practical applications in data privacy within the shuffle model of DP:

% \begin{itemize}
% \item From a theoretical standpoint, we have developed a new parameterization approach and sophisticated techniques for dissecting privacy amplification bounds, as elaborated in Section 5. These bounds represent a notable leap forward from current methodologies, especially in enhancing privacy-utility trade-offs for complex SQL queries.

% \item Practically, our work includes the development of a scalable $\tilde{O}(n)$ numerical algorithm designed for unified and tight privacy amplification analysis. This algorithm applies to all LDP, local metric DP and most of multi-message protocols. It directly improve the privacy-utility-message complexity trade-offs of shuffle protocols, and fills a critical gap in multi-message shuffle model researches (which provide no numerical method for tight privacy accounting), paving the way for its application beyond theoretical computer science areas (e.g., in \cite{erlingsson2019amplification,balle2019privacy,feldman2022hiding,feldman2023stronger}) to diverse application fields such as database/data mining, mobile/edge computing, and federated learning.
% \end{itemize}



% \begin{mybox}{Meta Reviewer-Item 4}
% Please add more explanations on the connection between this paper’s contribution and the interests of DB community.
% \end{mybox}

% One major goal of database is collecting, managing and analyzing user data. When these data are sensitive, some sort of privacy preserving techniques have to be integrated into the procedures of DB workflow. To this end,  tremendous works have contributed to this topic within the classical curator and local models of DP (as now added to the first paragraph of Section 1 Intoroduction, where most literatures are selected from top database/data science venues like VLDB and SIGMOD):
% \begin{quote}
% Specifically, tremendous works contribute to data collecting and analyses with curator model of DP (e.g., for count queries [ 18 , 19 , 56, 57 ], data mining [15 , 47 , 59 ], and general SQL engines [49, 55 ]) and local model of DP (e.g., for histogram query [ 9, 50 ], range query [23 , 25 , 69 ], marginal query [22 , 91 , 92], frequent  temset mining [83 , 86 ] and machine learning [26, 72, 74, 75]).
% However, curator model relies on unrealistic security assumptions (e.g., a fully trustable database), while the local model is long be criticized for low utility and restricts its realworld applications. This motivates and stimulates the emerging of shuffle DP model (which has its applications in Google \& Apple's Exposure Notification Privacy-preserving Analytics). The users can utilize an semi-trustable message shuffling party (e.g., anonymous channels, several non-colluding assistant parties with TEE) to anonymize their messages and hide among a message pool, before forwarding them to databases. Since messages are anonymized and randomly shuffled, each user only need to add more gentle noises (compared to the local DP) to gurantee to higher level of DP on shuffled messages. This is refer to as privacy amplification via shuffling.
% \end{quote}

% This work largely advances the critical component in the shuffle model: analyzing privacy amplification via shuffling, in terms of both tightness, usability and efficiency. The proposed framework is exactly tight for many LDP and multi-message shuffle protocols, and is extremely fast even when the number of users are billions. Therefore, it can directly improve the privacy-utility trade-offs in the local model (e.g., in [9, 50, 23 , 25 , 69, 22 , 91 , 92, 83 , 86, 26, 72, 74, 75]), and can guide the design of new multi-message protocols in the shuffle model (with much less message complexity). The efficiency of the framework making it suitable for large scale settings (e.g., collecting and analyzing sensitive data from millons or billions of users).

% Additionally, we present in-detail analyses of parallel local randomizers in Section 6, which are widely adopted in DB communities for privacy preservinghistogram queries, range queries, heavy-hitters identification, frequent itemset mining, decision trees. We also present related experimental results in Section 7.3 (specifically for a common SQL query: range query), and demonstrate significant utiltiy improvements.

% In summary, this work pioneers the study of collecting and analyzing large scale user data for DB community with newly emerging privacy preserving techniques. With the algoirhtms and tools provided by our work, one can achieve 
% (1) much better privacy-utility trade-offs, and
% (2) much less communication/compution costs 
% for aforementioned histogram queries, range queries, marginal queries, frequent itemset mnining, and machine learning over sensitive user data, thus making decentralized data collecting/analyses significantly more practical. Besides these direct implications, it has potential applications to multi-party (vertical) data collecting/analyzing cases, graph data collecting and analytics, and streaming data collecting, which are hot topics in the area of DB with data privacy preservation.

\begin{mybox}{Meta Reviewer-Item 4}
Please add more explanations on the connection between this paper’s contribution and the interests of DB community.
\end{mybox}

We recognize the importance of contextualizing our work within the interests of the DB community. Our research intersects significantly with key objectives in database management, particularly in the realm of sensitive user data handling:

Databases primarily focus on collecting, managing, and analyzing user data. When dealing with sensitive information, integrating privacy-preserving techniques into DB workflows is crucial. Our work advances this goal by building upon the foundational curator and local models of DP, as now detailed in the first paragraph of Section 1 Introduction. We reference key literature (i.e. count queries \cite{chen2011publishing,chen2014correlated,li2014data,li2015matrix}, data mining \cite{hu2015differential,bonomi2013mining,liu2021projected}, and general SQL engines \cite{johnson2018towards,kotsogiannis2019privatesql} in the curator DP model, histogram query \cite{kairouz2016discrete,bao2021cgm}, range query \cite{2019answering,du2021ahead,ren2022ldp}, marginal query \cite{cormode2018marginal,xu2019dpsaas,xu2020collecting}, frequent itemset mining \cite{wang2018locally,wang2020set} and machine learning \cite{duchi2013local,wang2018empirical,wang2019sparse,truex2020ldp} in the local DP model), from top database/data science venues like VLDB and SIGMOD to illustrate this.

However, existing models like the curator model, which relies on fully trustable databases, and the local model, known for low utility, have limitations. This has led to the rise of the shuffle DP model, as exemplified by its application in federated SQL queries~\cite{balle2020private,ghazi2020fewer,ghazi2021differentially,feldman2022hiding,cheu2022differentially}, federated machine learning~\cite{girgis2021shuffled,girgis2021shuffledtradeoffs,tenenbaum2021differentially,garcelon2022privacy}, and in Google \& Apple's Exposure Notification Privacy-preserving Analytics. The shuffle model employs semi-trustable shuffling parties for message anonymization, allowing users to add less noise compared to local DP for higher DP levels.

Our work significantly enhances the shuffle model's core aspect - analyzing privacy amplification via shuffling - in terms of tightness, usability, and efficiency. It is particularly effective for LDP and multi-message shuffle protocols, offering scalability even with billions of users. This directly improves privacy-utility trade-offs in local models and guides the design of new multi-message protocols in the shuffle model, reducing message complexity and increasing efficiency for large-scale data collection and analysis.

Furthermore, our in-depth analysis of parallel local randomizers in Section 6 and the experimental results in Section 7.3 (specifically for common SQL queries like range queries) demonstrate substantial utility improvements.

In summary, our work pioneers new methodologies for collecting and analyzing large-scale user data with emerging privacy-preserving techniques in the DB community. It offers:
\begin{itemize}
\item Enhanced privacy-utility trade-offs in sensitive user data collecting/analyzing,
\item Reduced communication and computation costs for various decentralized DB queries under privacy constraints,
\end{itemize}
thus rendering decentralized data collection and analysis more practical. Beyond these direct implications, our work has potential applications in multi-party data collection/analysis, graph data analytics, and streaming data collection, all of which are current hot topics in DB with a focus on data privacy preservation.




% \begin{mybox}{Meta Reviewer-Item 5}
% The presentation needs an improvement.
% \end{mybox}


% Thanks for the advice, we have thoroughly proofread the manuscript and optimize the entire introduction section.

\begin{mybox}{Meta Reviewer-Item 5}
The presentation needs an improvement.
\end{mybox}

In response to the reviewers' suggestion, we have carefully made the following adjustments to improve the presentation:
\begin{itemize}
\item An extensive proofreading exercise has been carried out to polish the manuscript and ensure linguistic precision.
\item The Introduction section has been overhauled to better articulate our research aims, the significance of our work, and its relevance to the field.
\item We have restructured certain paragraphs for better logical flow and reader engagement, ensuring that key arguments and findings are presented more coherently.
\end{itemize}
These refinements aim to enhance the manuscript's academic rigor and increase its attractiveness to readers.

\clearpage
\section*{Response to Reviewer \#3}


\begin{mybox}{Reviewer \#3-D1}
Overall, this paper provides improved results for shuffle DP that seems significant enough. Although the overall analysis follows existing 'hiding among clones'/'privacy blanket' pipeline, this paper introduces new techniques to obtain improved results.
\end{mybox}

We would like to thank you for the recognition of our contributions and for raising this issue. Besides the comparative summary in Section 2 Related Work, we now slightly revised the discussion on comparison with the closely related clone reduction in Section 4.1 as follows:
\begin{quote}
\textbf{Discussion on differences with  stronger clone reduction. } For $\epsilon_0$-LDP randomizers where $p\equiv q=\exp(\epsilon_0)$, our intermediate result presented in Theorem \ref{the:reduction} yields a divergence upper bound analogous to the one found in the state-of-the-art stronger clone by \cite{feldman2023stronger}. Our framework offers three primary advantages:
(i) Our bound is tighter than \cite{feldman2023stronger} as long as the newly introduced total variation parameter $\beta$ is not the worst-case $(p-1)/(p+1)$. Notably, commonly-used randomizers exhibit much lower $\beta$ values, and computing $\beta$ is straightforward.
(ii) While \cite{feldman2023stronger} handles only LDP randomizers that $q\equiv p$, our reduction is versatile, accommodating also cases where $p<q$ (e.g., for metric local randomizers) and $p>q$ (e.g., for multi-message randomizers).
(iii) Our method entails a $\tilde{O}(n)$-time algorithm for numerically determining the Hockey-stick divergence, offering a much more efficient solution compared to prevailing algorithms \cite{feldman2022hiding,koskela2021tight}, being about $10$ times faster than their documented execution times. Besides, to the best of knowledge, our work presents the first efficient numerical amplification method for multi-message shuffle protocols, thus can significantly boost the practicalness of them \cite{balcer2020separating,balcer2021connecting,cheu2022differentially,luo2022frequency,li2023privacy}.  
\end{quote}




\begin{mybox}{Reviewer \#3-D2}
The paper can be made easier to follow by providing more intuitions. For example, the intuition of introducing and decoupling based on the total variation bounds of local messages and the probability ratio bounds of blanket messages.
\end{mybox}

% Thanks for the insightful suggestion. For characterizing more precise mixture decoupling of randomizers in the shuffle model, we strive simple indicates/parameterizations that that reflects the (1) the statistical similarity/distance of the victim's outputs given two different inputs; (2) the mimic/clone capability of messages from other users. For the first target, when local randomizers having extremal probability design, though they are many possible distance measures, the total variation distance is a sufficient statistics. For the second target, the mixture decoupling mainly concerns with relative (instead of absolute) probability relations, thus is natural to introduce the $q$-ratio property among randomizers. We now add more intuitive about these parameterization for shuffle privacy amplification at the start of Section 4:

Thank you for your valuable suggestion. To enhance clarity, we now include additional intuitive explanations at the beginning of Section 4. Our approach for a more precise mixture decoupling of randomizers in the shuffle model involves straightforward indicators that reflect (1) the statistical similarity/distance of a victim's outputs given different inputs, and (2) the mimic/clone capability of messages from other users. Specifically, when dealing with local randomizers featuring extremal probability designs, the total variation distance emerges as a sufficient statistic for the first target. For the second target, as mixture decoupling primarily concerns relative probability relations, the introduction of the \(q\)-ratio property among randomizers becomes a natural choice. These intuitive explanations aim to provide a clearer understanding of our parameterizations for shuffle privacy amplification.


\begin{quote}
Our approach leverages the mixture decomposition of local randomizers, as introduced in the privacy blanket \cite{balle2019privacy} and clone reduction \cite{feldman2022hiding,feldman2023stronger} literature. The mixture decomposition of local randomizers reveal two important facts: (1) randomized and anonymously shuffled messages from other users can mimic as the message from a particular (victim) user with some probability, which are termed as blanket messages in \cite{balle2019privacy} and clones in \cite{feldman2022hiding,feldman2023stronger} and can thus amplify privacy; (2) for the local randomizer of the victim user that pertain to some properties (e.g., $(\epsilon,0)$-LDP), the probability distribution of outputs given arbitrary inputs share some resemblance. The key to analyzing tighter shuffle privacy amplification would be characterizing more concise mimic probability from other users and the probability resemblance of the victim's outputs. Compared to existing results, our framework achieves a highly precise mixture decomposition by utilizing both $(0,\delta)$-LDP and $(\epsilon_0, 0)$-LDP properties of local randomizers to capture the the probability resemblance of victim's outputs (over differed inputs), and introduces the probability ratio as simple yet effective indicates to the mimic power from other users.
\end{quote}



\begin{mybox}{Reviewer \#3-D3}
There are some typos need to be fixed. For example

Page 3: "Substituting the dataset $S$ in Definition 3.4 with with an individual data item": remove "with".

Page 9: "A more effective approach is to allow each user to randomly choose one query from among all K queries using a fixed probability distribution": remove "from" or "among".
\end{mybox}

Thank you for pointing out these typos. They have been corrected, and we have thoroughly reviewed the manuscript for any additional typos.

\clearpage
\section*{Response to Reviewer \#4}


\begin{mybox}{Reviewer \#4-W1}
The presentation of the paper is more suitable for a theory conference, it may help to provide a more accessible organization for a broader audience.
\end{mybox}

% Thanks for the overall strong positive feedback on our contribution. To increase the accessibility to broader audience like DB communities, we now have thorough rewrite the Section 1 Introduction, and add more intuition about our theoretical techniques and results in Section 4 and Section 5.

Thank you for the overall positive feedback and your suggestion for broadening the paper's accessibility. In response, we have undertaken a substantial rewrite of Section 1 (Introduction) to make it more comprehensible to a wider audience, including those in the DB community. Additionally, we have infused Sections 4 and 5 with more intuitive explanations of our theoretical techniques and results, aiming to bridge the gap between theoretical rigor and practical understanding.



\clearpage
\section*{Response to Reviewer \#5}


\begin{mybox}{Reviewer \#5-W1}
The scope of this work is narrowly defined. The manuscript focuses on the shuffle model of differential privacy and aims at deriving tighter privacy bournds for known randomizers and protocols.
\end{mybox}


% We appreciate the opportunity to clarify the scope and significance of our work. The shuffle model of differential privacy (DP), an emerging paradigm in comparison to the traditional curator and local models, has shown promising applications in diverse fields, such as SQL queries \cite{balle2020private,ghazi2020fewer,ghazi2021differentially,feldman2022hiding,cheu2022differentially}, federated learning \cite{girgis2021shuffled,girgis2021shuffledtradeoffs}, bandit learning \cite{tenenbaum2021differentially,garcelon2022privacy}, and in major projects like Google \& Apple's Exposure Notification Privacy-preserving Analytics. Its rapid adoption, extending beyond theoretical research into practical applications like database queries, information security, and machine learning, highlights its broad potential. Consequently, its extensive applications necessitate a unified, tight, and efficient framework for removing barriers in analyzing shuffle protocols (from theorists' perspectives) and in designing/implementing shuffle protocols (from practitioner's views).






% The most important and challenging part of the increasing popular shuffle model of DP is the analysis of privacy amplification via shuffling (as explored in significant works \cite{erlingsson2019amplification,balle2019privacy,feldman2022hiding,feldman2023stronger} from top venues). This analysis is distinct from the classical local and curator models of DP. Our contributions significantly enhance shuffle privacy amplification analysis, impacting both theory and practice:

% %
% %We thank the reviewer for the opportunity to further clarify the scope and significance of our work. The shuffle model of differential privacy (DP), an emerging paradigm in comparison to the traditional curator and local models, has shown promising applications in diverse fields, such as SQL queries \cite{balle2020private,ghazi2020fewer,ghazi2021differentially,feldman2022hiding,cheu2022differentially}, federated learning \cite{girgis2021shuffled,girgis2021shuffledtradeoffs}, bandit learning \cite{tenenbaum2021differentially,garcelon2022privacy}, and in major projects like Google & Apple's Exposure Notification Privacy-preserving Analytics. Its rapid adoption, extending beyond theoretical research into practical applications like database queries, information security, and machine learning, highlights its broad potential. Consequently, its extensive applications necessitate a unified, tight, and efficient framework for analyzing and designing shuffle protocols, both from theoretical and practical perspectives.

% % A key challenge in the increasingly popular shuffle model of DP is privacy amplification analysis via shuffling, as explored in significant works \cite{erlingsson2019amplification,balle2019privacy,feldman2022hiding,feldman2023stronger} from top venues. This analysis is distinct from the classical local and curator models of DP. Our contributions significantly enhance shuffle privacy amplification analysis, impacting both theory and practice:


% For theorists:
% \begin{itemize}
% \item Our innovative proof techniques, such as leveraging the total variation parameter for mixture decomposition (Lemma A.2), lead to precisely tight decompositions for various randomizers and potential multi-level extensions (see Appendix's Limitations section).
% \item We achieve qualitative advancements over existing LDP results (Table 1) and broaden the scope to multi-message scenarios, which are critical for improved utility.
% 3. New methodologies for establishing lower bounds in shuffle privacy amplification are introduced, enriching theoretical understanding.
% \end{itemize}

% For practitioners:
% \begin{itemize}
% \item The refined numerical amplification results we offer will directly enhance the privacy-utility trade-offs in existing applications, especially in large-scale data collection scenarios.
% \item Our work fills a gap in multi-message shuffle protocols by providing computational methods for privacy amplification, as evidenced in Table 2. This narrows the gap with centralized DP and improves overall protocol efficacy.
% \item Lastly, our asymptotic amplification findings help protocol designers grasp and optimize their designs through simplified randomizer parameterizations.
% \end{itemize}


% Our work not only has direct applications to existing DP randomizers and protocols (e.g., for heavy hitter estimation \cite{qin2016heavy, bassily2017practical, wang2019locally}, multi-dimensional data publication \cite{ren2018lopub, wang2019collecting, wang2019answering}, frequent itemset mining \cite{wang2018locally}, range queries \cite{cormode2019answering}, marginal queries \cite{cormode2018marginal}, data synthesis \cite{zhang2018calm, wangT2019locally}, and machine learning \cite{jagannathan2009practical,xin2019differentially,fletcher2019decision}), but also can inspire new multi-message protocols, as discussed on Page 7 and in our generality analysis for multi-message shuffle protocols, which have state-of-the-art (SOTA) privacy-utility balances:


% % Our work not only have directly applications to existing DP randomizers and protocols  (e.g., for heavy hitter estimation \cite{qin2016heavy, bassily2017practical, wang2019locally}, multi-dimensional data publication \cite{ren2018lopub, wang2019collecting, wang2019answering}, frequent itemset mining \cite{wang2018locally}, range queries \cite{cormode2019answering}, marginal queries \cite{cormode2018marginal}, data synthesis \cite{zhang2018calm, wangT2019locally}, and machine learning \cite{jagannathan2009practical,xin2019differentially,fletcher2019decision}.), but also can motivate new multi-message protocols, as elaborated in Discussion on variation-ratio parameters at Page 7 and in the discussion of generality for shuffle protocols (which have SOTA privacy-utility balances):

% \begin{quote}
% \textbf{Discussion on variation-ratio parameters.} 
% The research on parameters \(p\), \(\beta\), and \(q\) shows patterns that help design protocols for the shuffle model.
% Single-message shuffle protocols that utilize $\epsilon_0$-LDP randomizers are limited to $q=p=e^{\epsilon_0}$. Therefore, the clone probability $2r=2\beta p/((p-1)q)$ decreases significantly with $\epsilon_0$, and larger population are required to achieve global $(\epsilon,\delta)$-DP. Randomization mechanisms with better utility in the local model often fully exploit privacy constraints and have larger total variation bounds $\beta$, resulting in weaker privacy amplification effects (e.g., comparing randomized response with binary RR on $2$ options). Multi-message shuffle protocols typically set $q<p$ or even $q\ll p$ to increase the clone probability and reduce the number of messages transmitted per user. For local metric $d_{\dom{X}}$-DP randomizers that handle large data domains, $d_{max}$ is often set relatively high, and thus $q\geq p$. When a global privacy target is given, they need to strike a balance between local data utility (which increases with $d_{max}$) and privacy amplification effects (which decrease with $d_{max}$).
% \end{quote}

% \begin{quote}
% \textbf{Discussion on the  generality of our framework for multi-message protocols. } We note that our framework applies to all single-message shuffle protocols with local $\epsilon$-DP or local metric DP randomizers. While for
% multi-message protocols in the shuffle model, based on the correlation between outputted messages, they can be primarily categorized into three main types:
% \begin{itemize}
%     \item[I.] The first type of multi-message shuffle protocols is achieved by invoking multiple single-message protocols. This is seen as in the Recursive protocol in \cite{balle2020private} and the utility-complexity balanced protocol in \cite{girgis2023distributed}.
%     \item[II.] The second type involves sending one input-dependent message and multiple independent blanket messages, as seen in \cite{balcer2020separating,balcer2021connecting,cheu2022differentially,luo2022frequency,li2023privacy}.
%     \item[III.] The third type involves sending multiple correlated messages per user. Protocols falling in this category include \cite{ghazi2020private,ghazi2021differentially} and the secret-sharing-style IKOS protocol in \cite{balle2020private}.
% \end{itemize}
% We also envision that there can be multi-message protocols that combines Types I and II, by invoking several protocols each is a multi-message one. Our variation-ratio framework is compatible with protocols categorized under Type I and/or Type II.    
% \end{quote}

% % In summary, our work not only have direct applications to existing privacy preserving  protocols for well-studied data collecting/analyzing topics, but also removed the key obstacle of the new model of DP when spreading to new topics in broad application domains (including privacy-related DB researches), and can motivate novel randomizers/protocols design therein.

% In summary, our work not only has direct applications to existing privacy-preserving protocols in well-established data collection/analysis tasks and  domains but also overcomes significant challenges (e.g., in generality, tightness, and efficiency) in the new model of DP, facilitating its expansion into broader application areas (including privacy-related DB research). Furthermore, our findings and methodologies can stimulate the development of innovative randomizers and protocols within these spreading domains.

We are grateful for the chance to elaborate on the impact and breadth of our research. The shuffle model of DP stands as a relatively new paradigm when compared to traditional curator and local models, yet it has already shown considerable promise across various applications. This includes advancements in SQL queries \cite{balle2020private,ghazi2020fewer,ghazi2021differentially,feldman2022hiding,cheu2022differentially}, federated learning \cite{girgis2021shuffled,girgis2021shuffledtradeoffs}, bandit learning \cite{tenenbaum2021differentially,garcelon2022privacy} and its deployment in major projects like Google \& Apple's Exposure Notification Privacy-preserving Analytics. Its swift integration into practical fields like database queries, information security, and machine learning underscores the model's vast applicability and potential. 
The expansive applications of the shuffle model necessitate an urgent development of a unified and efficient framework that addresses both the theoretical complexities of analyzing shuffle protocols and the practical challenges in their design and implementation, highlighting the critical needs of both theorists and practitioners.
%On the other hand, its broad applications call for a unified, tight, and fast framework for removing barriers in analyzing shuffle protocols (from theorists' perspectives) and in designing/implementing shuffle protocols (from practitioner's views).

The challenge of analyzing privacy amplification in the shuffle model of DP, as discussed in previous leading publications \cite{erlingsson2019amplification,balle2019privacy,feldman2022hiding,feldman2023stronger}, is pivotal. Nonetheless, existing works have not established sufficiently tight bounds for broader communication scenarios, limiting its applicability in real-world big data applications.
%The most important and challenging part of the increasing popular shuffle model of DP is the analyses of privacy amplification via shuffling (as pursued in a series of works \cite{erlingsson2019amplification,balle2019privacy,feldman2022hiding,feldman2023stronger} from top venues), which disguises itself from the classical local and curator models of DP. 

To summarize, we significantly enhanced the analysis of shuffle privacy amplification for the theorists and the practitioners:

For the theorists:
\begin{itemize}
\item Our innovative proof techniques, such as leveraging the total variation parameter for mixture decomposition (Lemma \ref{lemma:mixture}), lead to precisely tight decompositions for various randomizers and potential multi-level extensions.
\item We achieve qualitative advancements over existing LDP results (see Table \ref{tab:bounds}) and broaden the scope to multi-message scenarios, which are critical for improved utility.
\item New methodologies for establishing lower bounds in shuffle privacy amplification are introduced, enriching theoretical understanding.
\end{itemize}

For the practitioners:
\begin{itemize}
\item The refined numerical amplification results we offer will directly enhance the privacy-utility trade-offs in existing applications, especially in large-scale data collection scenarios.
\item Our work fills a gap in multi-message shuffle protocols by providing $\tilde{O}(n)$ computational methods for privacy amplification, as evidenced in Algorithm \ref{alg:upperbound} and Table \ref{tab:parametersmulti}. This narrows the gap with centralized DP and improves overall protocol efficacy.
\item Lastly, our asymptotic amplification findings help protocol designers grasp and optimize their designs through simplified randomizer parameterizations.
\end{itemize}

Our work not only has direct applications to existing DP randomizers and protocols  (e.g., for heavy hitter estimation \cite{qin2016heavy, bassily2017practical, wang2019locally}, multi-dimensional data publication \cite{ren2018lopub, wang2019collecting, wang2019answering}, frequent itemset mining \cite{wang2018locally}, range queries \cite{cormode2019answering}, marginal queries \cite{cormode2018marginal}, data synthesis \cite{zhang2018calm, wangT2019locally}, and machine learning \cite{jagannathan2009practical,xin2019differentially,fletcher2019decision}.), but also can motivate new multi-message protocols, as elaborated in Discussion on variation-ratio parameters at Page 8 and in the discussion of generality for shuffle protocols (which have best privacy-utility balances):

\begin{quote}
\textbf{Discussion on variation-ratio parameters.} 
The research on parameters \(p\), \(\beta\), and \(q\) shows patterns that help design protocols for the shuffle model.
Single-message shuffle protocols that utilize $\epsilon_0$-LDP randomizers are limited to $q=p=e^{\epsilon_0}$. Therefore, the clone probability $2r=2\beta p/((p-1)q)$ decreases significantly with $\epsilon_0$, and larger population are required to achieve global $(\epsilon,\delta)$-DP. Randomization mechanisms with better utility in the local model often fully exploit privacy constraints and have larger total variation bounds $\beta$, resulting in weaker privacy amplification effects (e.g., comparing randomized response with binary RR on $2$ options). Multi-message shuffle protocols typically set $q<p$ or even $q\ll p$ to increase the clone probability and reduce the number of messages transmitted per user. For local metric $d_{\dom{X}}$-DP randomizers that handle large data domains, $d_{max}$ is often set relatively high, and thus $q\geq p$. When a global privacy target is given, they need to strike a balance between local data utility (which increases with $d_{max}$) and privacy amplification effects (which decrease with $d_{max}$).
\end{quote}

\begin{quote}
\textbf{Discussion on the generality of our framework for multi-message protocols. } We note that our framework applies to all single-message shuffle protocols with local $\epsilon$-DP or local metric DP randomizers. While for multi-message protocols in the shuffle model, based on the correlation between outputted messages, they can be primarily categorized into three main types:
\begin{itemize}
    \item[I.] The first type of multi-message shuffle protocols is achieved by invoking multiple single-message protocols. This is seen as in the Recursive protocol in \cite{balle2020private} and the utility-complexity balanced protocol in \cite{girgis2023distributed}.
    \item[II.] The second type involves sending one input-dependent message and multiple independent blanket messages, as seen in \cite{balcer2020separating,balcer2021connecting,cheu2022differentially,luo2022frequency,li2023privacy}.
    \item[III.] The third type involves sending multiple correlated messages per user. Protocols falling in this category include \cite{ghazi2020private,ghazi2021differentially} and the secret-sharing-style IKOS protocol in \cite{balle2020private}.
\end{itemize}
We also envision that there can be multi-message protocols that combines Types I and II, by invoking several protocols each is a multi-message one. Our variation-ratio framework is compatible with protocols categorized under Type I and/or Type II.    
\end{quote}

In summary, our work not only have direct applications to existing privacy preserving  protocols for well-studied data collecting/analyzing topics, but also removed the key obstacle of the new model of DP when spreading to new topics in broad application domains (including privacy-related DB researches), and can motivate novel randomizers/protocols design therein.



\begin{mybox}{Reviewer \#5-W2}
Contribution/result of this work is theoretical. There is no new development of algorithms in this work.
\end{mybox}

We thank the reviewers for recognizing our theoretical contributions. Our research also significantly improves practical applications by ensuring large databases maintain functionality after Differential Privacy (DP) implementation. This advancement supports sectors like database/data mining, mobile/edge computing, and federated learning (e.g., in \cite{erlingsson2019amplification,balle2019privacy,feldman2022hiding,feldman2023stronger}), which require complex SQL queries with minimal added noise. Previously, the lack of a scalable \(\tilde{O}(n)\) numerical algorithm for comprehensive and precise privacy amplification analysis hindered these applications. Our research addresses this by improving the balance between privacy, utility, and message complexity in shuffle protocols, bridging a vital gap in multi-message shuffle model studies that lacked a numerical method for accurate privacy calculations.

As we mentioned in the previous response, the privacy amplification analysis lies in the heart of the shuffle model of DP, a burgeoning area in data privacy. There are plethora of randomizers/protocols available in the local DP literature, most shuffle protocols (e.g. \cite{balle2020private,ghazi2020fewer,ghazi2021differentially,feldman2022hiding,cheu2022differentially,girgis2021shuffled,girgis2021shuffledtradeoffs,tenenbaum2021differentially,garcelon2022privacy})  merely adapt them from the local model to the shuffle model. A critical and challenging aspect of this adaptation is understanding how these randomizers perform after anonymizing/shuffling (as an important part of \emph{shuffle DP algorithms}), a major concern for both theorists and practitioners.

%Numerous randomizers and protocols in the local DP literature (e.g., \cite{balle2020private,ghazi2020fewer,ghazi2021differentially,feldman2022hiding,cheu2022differentially,girgis2021shuffled,girgis2021shuffledtradeoffs,tenenbaum2021differentially,garcelon2022privacy}) have been adapted for the shuffle model. A critical and challenging aspect of this adaptation is understanding how these randomizers perform post-shuffling, a concern for both theorists and practitioners.

Our work significantly enhances the privacy amplification via shuffling, simultaneously improving generality (i.e. apply to all LDP, local metric DP randomizers, and most of multi-message protocols), tightness (i.e. saves significant privacy budget to achieve better privacy-utility-message complexity trad-offs), and computational efficiency (i.e. providing an $\tilde{O}(n)$ algorithm for amplifying privacy for large-scale applications).

Our work contributes to both the theoretical framework and practical applications in privacy preserving data collecting/analyzing within the shuffle model of DP:

\begin{itemize}
\item From a theoretical standpoint, we have developed a new parameterization approach and sophisticated techniques for dissecting privacy amplification bounds, as elaborated in Section 5. These bounds represent a notable leap forward from current methodologies, especially in enhancing privacy-utility trade-offs for complex SQL queries.

\item Practically, our work includes the development of a scalable $\tilde{O}(n)$ numerical algorithm designed for unified and tight privacy amplification analysis. This algorithm applies to all LDP, local metric DP and most of multi-message protocols. It directly improve the privacy-utility-message complexity trade-offs of shuffle protocols, and fills a critical gap in multi-message shuffle model researches (which provide no numerical method for tight privacy accounting), paving the way for its application beyond theoretical computer science areas (e.g., in \cite{erlingsson2019amplification,balle2019privacy,feldman2022hiding,feldman2023stronger}) to diverse application fields such as database/data mining, mobile/edge computing, and federated learning.
\end{itemize}


%the emerging shuffle model is reshaping the privacy preservation techniques for decentralized user data collecting and analyses, in the context of stringent data privacy regulations. This work focus on the most fundamental component of the shuffle model: analyzing the privacy amplification of shuffling, and contributes a more unified, tighter, and more efficient framework. 
